Unveiling the Potential of Structure Preserving for Weakly Supervised Object Localization

Weakly supervised object localization(WSOL) remains an open problem given the deficiency of finding object extent information using a classification network. Although prior works struggled to localize objects through various spatial regularization strategies, we argue that how to extract object structural information from the trained classification network is neglected. In this paper, we propose a two-stage approach, termed structure-preserving activation (SPA), toward fully leveraging the structure information incorporated in convolutional features for WSOL. First, a restricted activation module (RAM) is designed to alleviate the structure-missing issue caused by the classification network on the basis of the observation that the unbounded classification map and global average pooling layer drive the network to focus only on object parts. Second, we designed a post-process approach, termed self-correlation map generating (SCG) module to obtain structure-preserving localization maps on the basis of the activation maps acquired from the first stage. Specifically, we utilize the high-order self-correlation (HSC) to extract the inherent structural information retained in the learned model and then aggregate HSC of multiple points for precise object localization. Extensive experiments on two publicly available benchmarks including CUB-200-2011 and ILSVRC show that the proposed SPA achieves substantial and consistent performance gains compared with baseline approaches.Code and models are available at https://github.com/Panxjia/SPA_CVPR2021

==> Figures/err_alg.tex <==
\begin{algorithm}[htb]  
  \caption{ Error Analysis Algorithm.}  
  \label{alg:err_alg}  
  \begin{algorithmic}[1]  
    \Require  
      Predicted bounding box $B_{p} \in \mathbb{R}^{1 \times 4 }$; Predicted label $C_p$; ground truth boxes list $B_{g} \in \mathbb{R}^{N \times 4 }$; ground truth label $C_g$; 
      Maximum IoU $\hat{IoU}$ between the $B_{p}$ and $B_{g}$;
    \Ensure  
      Cls, M-Ins, Part, More, OT; 
    \State Set Cls = M-Ins = Part = More = OT = 0
    \If{$C_p \neq C_b[0]$}
        \State Cls =1
        \State \Return Cls, M-Ins, Part, More, OT
    \EndIf
    \If {$\hat{IoU} > 0.5$ }
        \State \Return Cls, M-Ins, Part, More, OT
    \EndIf 
    \State Calculate $IoG \in \mathbb{R}^{1 \times N }$ between the $B_{p}$ and $B_{g}$
    \If {$Count(IoG > 0.3) > 1 $}
        \State M-Ins = 1 
        \State \Return Cls, M-Ins, Part, More, OT
    \EndIf 
    \State Calculate the maximum $\hat{IoG}$ and $\hat{IoP}$
    \If {$ \hat{IoP} > 0.5$}
        \State Part = 1 
        \State \Return Cls, M-Ins, Part, More, OT
    \EndIf 
    \If {$\hat{IoG} > 0.7$}
        \State More = 1 
        \State \Return Cls, M-Ins, Part, More, OT
    \EndIf 
    \State OT = 1 
    \State \Return Cls, M-Ins, Part, More, OT
  \end{algorithmic}  
\end{algorithm}  

==> Figures/qualitative_sc2_rebuttal.tex <==
\begin{wrapfigure}[7]{r}{0.4\linewidth}
% \vspace{-8pt}
\centering
% \includegraphics[trim=2.8cm 0cm 0cm 1cm,width=\linewidth]{Images/qualitative_analysis_hsc.pdf}
\includegraphics[trim=2cm 5cm 0cm 1.5cm, width=\linewidth]{Images/qualitative_analysis_hsc.pdf}

\end{wrapfigure}

==> Figures/sup_hsc_0.tex <==
\begin{figure*}[!thb]
\centering
\includegraphics[width=0.95\linewidth]{Images/sup_hsc_0.pdf}
\caption{Visualization of the self-correlation maps with first-order similarity (middle row) and second-order similarity(bottom row).  The images are from the CUB-200-2011~\cite{wah2011caltech} testing set.}
\label{fig:sup_hsc_0}
\end{figure*}

==> Figures/sup_hsc_1.tex <==
\begin{figure*}[!thb]
\centering
\includegraphics[width=0.95\linewidth]{Images/sup_hsc_1.pdf}
\caption{Visualization of the self-correlation maps with first-order similarity (middle row) and second-order similarity(bottom row).  The images are from the CUB-200-2011~\cite{wah2011caltech} testing set.}
\label{fig:sup_hsc_1}
\end{figure*}

==> Figures/sup_hsc_2.tex <==
\begin{figure*}[!thb]
\centering
\includegraphics[width=0.95\linewidth]{Images/sup_hsc_2.pdf}
\caption{Visualization of the self-correlation maps with first-order similarity (middle row) and second-order similarity(bottom row).  The images are from the CUB-200-2011~\cite{wah2011caltech} testing set.}
\label{fig:sup_hsc_2}
\end{figure*}

==> Figures/sup_hsc_3.tex <==
\begin{figure*}[!thb]
\centering
\includegraphics[width=0.95\linewidth]{Images/sup_hsc_3.pdf}
\caption{Visualization of the self-correlation maps with first-order similarity (middle row) and second-order similarity(bottom row).  The images are from the ILSVRC~\cite{russakovsky2015imagenet} validation set.}
\label{fig:sup_hsc_3}
\end{figure*}

==> Figures/sup_res_0.tex <==
\begin{figure*}[!htb]
\centering
\includegraphics[width=0.95\linewidth]{Images/sup_res_0.pdf}
\caption{Visualization of the localization maps with CAM~\cite{zhou2016learning} (middle row) and the proposed SPA(bottom row).  The images are from the ILSVRC~\cite{russakovsky2015imagenet} validation set.}
\label{fig:sup_res_0}
\end{figure*}

==> Figures/sup_res_1.tex <==
\begin{figure*}[!htb]
\centering
\includegraphics[width=0.95\linewidth]{Images/sup_res_1.pdf}
\caption{Visualization of the localization maps with CAM~\cite{zhou2016learning} (middle row) and the proposed SPA(bottom row).  The images are from the ILSVRC~\cite{russakovsky2015imagenet} validation set.}
\label{fig:sup_res_1}
\end{figure*}

==> Figures/sup_res_2.tex <==
\begin{figure*}[!thb]
\centering
\includegraphics[width=0.95\linewidth]{Images/sup_res_2.pdf}
\caption{Visualization of the localization maps with CAM~\cite{zhou2016learning} (middle row) and the proposed SPA(bottom row).  The images are from the ILSVRC~\cite{russakovsky2015imagenet} validation set.}
\label{fig:sup_res_2}
\end{figure*}

==> Sections/sup.tex <==
\section{High-order Self Correlation}
To apply the inherent structure-preserving ability of the network for accurate WSOL, we propose to use high-order self-correlation (HSC) to capture the structural information of objects. 
The $h_{th}$ order similarity between $f_i$ and $f_i$ are formulated as:
\begin{small}
\begin{equation}
    S^{h}(f_i, f_j) = \frac{1}{(HW)^{h-1}}\sum_{k^{0} }\cdots \sum_{k^{h-2}}S(f_i, f_{k^{0}})\cdots S(f_{k^{h-2}},f_j),
\end{equation}
\end{small}
where $k^{0}, k^{h-2} \in \Omega$, $h \in \{2,3,4 \cdots \}$ and $i\neq k^{0} \neq k^{h-2}$. $h$ denotes the order, and $\Omega$ denotes the set of all features. 
The $S^{h}(f_i, f_j)$ is then normalized to $[0, 1]$ following:
\begin{equation}
    \hat{S}^{h}(f_i, f_j) = \frac{S^{h}(f_i, f_j) - min_{k \in \Omega}S^{h}(f_i, f_k) }{max_{k \in \Omega}S^{h}(f_i, f_k) - min_{k \in \Omega}S^{h}(f_i, f_k)},
\end{equation}
%We here show a second-order case, and one can easily extend to higher order.
Then, we define HSC as:
\begin{equation}
    %{Cor}^h = ReLU(S^{h}(f^{'\mathrm{T}}, f^{'}))
    {SC}^h(f) = \left [ \hat{S}^h(f_i, f_j) | _{i,j} \right ].
    \label{equ:ch}
\end{equation}
Compared with first-order self-correlation, HSC can preserve the details of the object by considering long-range context. 
However, the HSC may introduce additional noise.


\section{Quantitative Results}
\label{sec:sup}

\paragraph{Bounding Box Localization}
\inputtable{ilsvrc_main_sup}
\inputtable{cub_main_sup}
We here show more results on bounding boxes localization. Table~\ref{tab:ilsvrc_main_sup} and Table~\ref{tab:cub_main_sup} are the localization results on ILSVRC validation and CUB-200-2011 testing sets, respectively. 
On ILSVRC validation set, we achieve the state-of-the-art with VGG16, and obtain comparable results with current state-of-the-art method I$^{2}C$~\cite{zhang2020inter} with Inception V3.
Compared with baseline methods, the proposed SPA is much simpler and almost parameter-free without introducing additional convolutional layers.
On CUB-200-2011 testing set, the proposed SPA surpassing all the baseline methods.

\inputtable{err_analysis_sup}
\paragraph{Error Analysis.}
To further reveal the effect of our method, we define five metrics to perform bad case analysis on the proposed SPA approach.
Specifically, we divide the localization error into five cases: classification error (Cls), multi-instance error (M-Ins), localization part error (Part), localization more error (More), and others (OT).
For better description, we also define \emph{IoG} and \emph{IoP}.
Similar to \emph{IoU}(intersection over Union), IoG means that intersection over ground truth box and IoP means that intersection over predict bounding box.
\begin{itemize}
    \item \emph{Cls} includes the predictions that are wrongly classified.
    \item \emph{M-Ins} indicates that the prediction intersects with at least two ground truth boxes, and IoG $>$ 0.3.
    \item \emph{Part} indicates that the predicted bounding box only cover the parts of object, and IoB $>$ 0.5.
    \item \emph{More} indicates that the predicted bounding box is larger than the ground truth bounding box by a large margin, and IoG $>$ 0.7.
    \item \emph{OT} indicates other predictions that do not fall under above mentioned cases.
\end{itemize}
The five cases defined above are mutually exclusive. We show the details of the definition of five metrics in Algorithm~\ref{alg:err_alg}
\inputfigure{err_alg}
Each metric calculates the percentage of images belonging to corresponding error in the validation/testing set.
Table~\ref{tab:err_analysis_sup} lists localization error statistics.
Localization error \emph{Cls} caused by wrong classification dominates the error. But the classification is not the main concern for WSOL.
We mainly focus on \emph{M-Ins}, \emph{Part}, and \emph{More} metrics.
For ILSVRC, the proposed SPA effectively reduces the three kinds of localization error.
Although there is no explicit solution for multi-instance problem, our method reduces the \emph{M-Ins} error.
From Table~\ref{tab:err_analysis_sup}, it shows that the \emph{M-Ins} and \emph{More} are the most important problems to solve.
It it worth to explore CAM-based methods for \emph{weakly supervised instance localization} in future work.  
For CUB-200-2011, there is only one instance in each image.
Our method effectively reduces \emph{Part} and \emph{More} errors on VGG16, which indicates that our localization maps are much accurate.
On Inception V3, the proposed SPA significantly reduce \emph{Part} by 10.2$\%$. 

\section{More Examples}
\inputfigure{sup_hsc_0}
\inputfigure{sup_hsc_1}
\inputfigure{sup_hsc_2}
\inputfigure{sup_hsc_3}
\paragraph{Self-correlation Maps.}
We here show more visualization examples for self-correlation maps in Fig.~\ref{fig:sup_hsc_0}, Fig.~\ref{fig:sup_hsc_1}, Fig.~\ref{fig:sup_hsc_2}, Fig.~\ref{fig:sup_hsc_3}.
In each figure, we show five self-correlation maps for corresponding points marked by green cross in original images.
The middle row shows the first-order self-correlation maps and the bottom row shows the second-order self-correlation maps.

\inputfigure{sup_res_0}
\inputfigure{sup_res_1}
\inputfigure{sup_res_2}
\paragraph{localization Results.}
We also show more visualization examples of localization maps in Fig.~\ref{fig:sup_res_0}, Fig.~\ref{fig:sup_res_1}, Fig.~\ref{fig:sup_res_2}.
In each figure, the original images with ground truth bounding boxes (in red) are shown in top row.
The localization maps with CAM and the proposed SPA are shown in middle and bottom row, respectively.

\paragraph{Ablation study of $\tau$ and $\sigma$ in Equs.~3 and 4.} $M_{bg}$ and $M_{obj}$ are calculated by Equs.~3 and 4 under different $\tau$s and $\sigma$s. Average mask IoU, IoG (Intersection over GT), and IoP (Intersection over Prediction) are reported in Table~\ref{tab:sup_ablation}. 
One can see that larger IoG implies the generated masks covering most of the desired region while low IoP means most of the masks are corrected. As the initial masks, $M_{bg}$ and $M_{obj}$, are good enough to guide the model to suppress backgrounds and active full object extent, statistically. 

\paragraph{Ablation study of $\alpha$, $\tau$ and $\sigma$.} We fix two of these variables and report the results with the variety of the left one on ILSVRC in Tables~\ref{tab:sup_abl_alpha}, \ref{tab:sup_abl_tau} and \ref{tab:sup_abl_sigma}. 


\inputtable{ilsvrc_vgg_rebuttal}

==> Tables/cub_main_sup.tex <==
\begin{table*}%[h]
\centering
%\resizebox{.48\textwidth}{!}{
\setlength{\tabcolsep}{2.8mm}{
\begin{tabular}{l|c|c|c|c|c|c}
	\toprule
      \multirow{2}{*}{Methods} &\multirow{2}{*}{Backbone}  &\multicolumn{3}{|c|}{Loc Err.} & \multicolumn{2}{|c}{Cls Err.}  \\ 
      \cline{3-7}
       &  &Top-1 & Top-5&Gt-Known &Top-1 &Top-5 \\ \hline
       CAM~\cite{zhou2016learning} & GoogLeNet~\cite{szegedy2015going} & 58.94 & 49.34 &44.9 & 26.2 &8.5 \\
       SPG~\cite{zhang2018self} & GoogLeNet~\cite{szegedy2015going} & 53.36 &42.8 & - &- &- \\
       DANet~\cite{xue2019danet} & InceptionV3~\cite{szegedy2016rethinking} & 50.55 &39.54 & 33.0 & 28.8 & 9.4 \\
       ADL~\cite{choe2019attention} & InceptionV3~\cite{szegedy2016rethinking} & 46.96 & - & - & {\bf 25.45} & - \\ 
       Ours & InceptionV3~\cite{szegedy2016rethinking} & {\bf 46.41} &{\bf 33.50} &{\bf 27.86}  & 26.49 & 8.61 \\ \hline
       CAM~\cite{zhou2016learning} & VGG16~\cite{simonyan2014very} &55.85 &47.84 &44.0 &{\bf 23.4} & {\bf 7.5} \\
       ADL~\cite{choe2019attention} & VGG16~\cite{simonyan2014very} & 47.64 & -&-&34.73&- \\
       ACoL~\cite{zhang2018adversarial} &VGG16~\cite{simonyan2014very} &54.08 &43.49 & 45.9 &28.1 &- \\
       DANet~\cite{xue2019danet} &VGG16~\cite{simonyan2014very} &47.48 &38.04 & 32.3 & 24.6 & 7.7 \\
       SPG~\cite{zhang2018self} & VGG16~\cite{simonyan2014very} & 51.07 &42.15 & 41.1 & 24.5 & 7.9 \\
       I$^{2}$C~\cite{zhang2020inter} & VGG16~\cite{simonyan2014very} &44.01 &31.6 & - &- &- \\
       MEIL~\cite{mai2020erasing} &VGG16~\cite{simonyan2014very} &42.54 & - & - &25.23 &- \\
       %GC-Net~\cite{lu2020geometry} &VGG16 & {\bf 36.76} & {\bf 24.46} &{\bf 18.9} & {\bf 23.2} & {\bf 7.7} \\
       Ours & VGG16~\cite{simonyan2014very} & {\bf 39.73} & {\bf 27.5} &  {\bf22.71} & 23.89 & 7.85 \\
	\bottomrule
\end{tabular}
\caption{Comparison between our method and the state-of-the-art on the CUB-200-2011 test set. Here ‘ClsErr’, ‘LocErr’ and ’Gt-Known’ are short for classification error, location error and Gt-known location error, respectively.}
\label{tab:cub_main_sup}
}
%}
\end{table*}

==> Tables/err_analysis_sup.tex <==
\begin{table*}[!h]
\centering
% \resizebox{.98\textwidth}{!}{
\setlength{\tabcolsep}{3.2mm}{
\begin{tabular}{l|ccccc|ccccc}
	\toprule
    \multirow{2}{*}{Methods} &\multicolumn{5}{|c}{ILSVRC($\%$)}  &\multicolumn{5}{|c}{CUB-2011-200($\%$)} \\
     &Cls&M-Ins & Part & More &OT & Cls &M-Ins & Part &More & OT\\
    \hline
    VGG16 &29.47 &10.65 &3.85 &9.58&0.2 &23.28 &- &21.91 &10.53&1.76 \\
     Ours &29.49 & 9.97& 2.83 &7.66 &0.5 &23.89 &-  & 9.25 &6.33&0.26 \\
    \hline
    InceptionV3 &26.73 &10.36 &3.22 &9.49&0.20 &26.39 &- &23.09&5.52&0.64 \\
     Ours &26.74 &9.48  & 2.89 &7.80 &0.37 &26.49 &-  &12.81  &6.83&0.03  \\
	\bottomrule
\end{tabular}
}
\caption{Localization error statistics.}
\label{tab:err_analysis_sup}
%}
\end{table*}

==> Tables/eval_var_rebuttal_bg.tex <==
\begin{table}%[h]
\centering
\resizebox{.24\textwidth}{!}{
\begin{tabular}{c|c|c|c||c|c|c|c}
	\toprule
   $\tau$(bg) & $IoU$ & $IoG$ & $IoP$ & $\tau$ + $\sigma$(fg) & $IoU$ & $IoG$ & $IoP$ \\ \hline
    0.1 & 0.42 & 0.44 & 0.92 & 0.0 &0.30 & 1.00 & 0.30 \\
    0.2 & 0.54 & 0.59 & 0.89 & 0.1 &0.33 & 1.00 & 0.33 \\
    0.3 & 0.60 & 0.69 & 0.86 & 0.2 &0.36 & 0.99 & 0.35 \\
    0.4 & 0.65 & 0.77 & 0.83 & 0.3 &0.37 & 0.98 & 0.37 \\
    0.5 & 0.67 & 0.83 & 0.80 & 0.4 &0.38 & 0.97 & 0.38 \\
    0.6 & 0.69 & 0.87 & 0.77 & 0.5 &0.38 & 0.95 & 0.40 \\
    0.7 & 0.69 & 0.90 & 0.76 & 0.6 &0.38 & 0.93 & 0.41 \\
    0.8 & 0.70 & 0.92 & 0.76 & 0.7 &0.39 & 0.90 & 0.43 \\
    0.9 & 0.71 & 0.94 & 0.75 & 0.8 &0.39 & 0.86 & 0.34 \\
    % 0.1 & 0.45 & 0.46 & 0.99 & 0.0 &0.16 & 1.00 & 0.16 \\
    % 0.2 & 0.58 & 0.58 & 0.98 & 0.1 &0.19 & 1.00 & 0.19 \\
    % 0.3 & 0.65 & 0.67 & 0.98 & 0.2 &0.21 & 1.00 & 0.21 \\
    % 0.4 & 0.71 & 0.73 & 0.96 & 0.3 &0.23 & 0.99 & 0.23 \\
    % 0.5 & 0.76 & 0.79 & 0.95 & 0.4 &0.24 & 0.98 & 0.24 \\
    % 0.6 & 0.78 & 0.84 & 0.93 & 0.5 &0.25 & 0.98 & 0.26 \\
    % 0.7 & 0.80 & 0.86 & 0.92 & 0.6 &0.27 & 0.98 & 0.27 \\
    % 0.8 & 0.82 & 0.89 & 0.91 & 0.7 &0.28 & 0.97 & 0.29 \\
    % 0.9 & 0.83 & 0.91 & 0.91 & 0.8 &0.30 & 0.95 & 0.31 \\
	\bottomrule 
\end{tabular}
}
% \caption{IoG:Intersection over Ground Truth, IoP: Intersection over Prediction.}
\label{tab:eval_var_reb}
\end{table}

==> Tables/ilsvrc_main_sup.tex <==
\begin{table*}[!th]
\centering
%\resizebox{.48\textwidth}{!}{
\setlength{\tabcolsep}{3.2mm}{
\begin{tabular}{l|c|c|c|c|c|c}
	\toprule
      \multirow{2}{*}{Methods} &\multirow{2}{*}{Backbone}  &\multicolumn{3}{|c|}{Loc Err.} & \multicolumn{2}{|c}{Cls Err.}  \\ 
      \cline{3-7}
       &  &Top-1 & Top-5&Gt-Known &Top-1 &Top-5 \\ \hline
       Backprop~\cite{simonyan2013deep} & VGG16~\cite{simonyan2014very} & 61.12 & 51.46 & - & - & - \\
       CAM~\cite{zhou2016learning} & VGG16~\cite{simonyan2014very} &57.20 &45.14 &- &31.2 & 11.4 \\
       CutMix~\cite{yun2019cutmix} & VGG16~\cite{simonyan2014very} &56.55 &- & - &- & - \\
       ADL~\cite{choe2019attention} & VGG16~\cite{simonyan2014very} & 55.08 & -&-&-&- \\
       ACoL~\cite{zhang2018adversarial} &VGG16~\cite{simonyan2014very} &54.17 &40.57 & 37.04 &32.5&12.0 \\
       I$^{2}$C~\cite{zhang2020inter} & VGG16~\cite{simonyan2014very} &52.59 &41.49 & 36.10 &30.6&10.7 \\
       MEIL~\cite{mai2020erasing} &VGG16~\cite{simonyan2014very} &53.19 & - & - &29.73 &- \\
       Ours & VGG16~\cite{simonyan2014very} &{\bf 50.44} &{\bf 38.68} & {\bf 34.95} &{\bf 29.49} & {\bf 9.95} \\ \hline
       CAM~\cite{zhou2016learning} &InceptionV3~\cite{szegedy2016rethinking} &53.71 & 41.81 &37.32 &26.7 & 8.2 \\
       SPG~\cite{zhang2018self} & InceptionV3~\cite{szegedy2016rethinking} &51.40 & 40.00 & 35.31 & 30.3 & 9.9 \\
       ADL~\cite{choe2019attention} &InceptionV3~\cite{szegedy2016rethinking} &51.29 & - & - &27.2 & - \\
       ACoL~\cite{zhang2018adversarial} & GoogLeNet~\cite{szegedy2015going} & 53.28 & 42.58 & - &29.0 & 11.8 \\
       DANet~\cite{xue2019danet} &GoogLeNet~\cite{szegedy2015going} & 52.47 & 41.72 &- &27.5 &8.6 \\
       MEIL~\cite{mai2020erasing} &InceptionV3~\cite{szegedy2016rethinking} & 50.52 & - &- &26.69 &- \\
       I$^{2}$C~\cite{zhang2020inter} & InceptionV3~\cite{szegedy2016rethinking} & {\bf 46.89} &35.87 & {\bf 31.50} & 26.7 & 8.4 \\
       GC-Net~\cite{lu2020geometry} & InceptionV3~\cite{szegedy2016rethinking} & 50.94 & 41.91 & - &{\bf 22.6} & {\bf 6.4} \\
       Ours &InceptionV3~\cite{szegedy2016rethinking} &47.29 & {\bf 35.73} &31.67 &26.74 &8.19 \\
	\bottomrule
\end{tabular}
}
\caption{Comparison between our method and the state-of-the-art on the ILSVRC~\cite{russakovsky2015imagenet} validation set. Our method outperforms all other methods by a large margin for object localization. Here ‘ClsErr’, ‘LocErr’ and ’Gt-Known’ are short for classification error, location error and Gt-known location error, respectively.}
\label{tab:ilsvrc_main_sup}
%}
\end{table*}

==> Tables/ilsvrc_vgg_alpha_abl.tex <==
% \begin{table}[!th]
% \centering
% \resizebox{.24\textwidth}{!}{
% % \setlength{\tabcolsep}{3.2mm}{
% \begin{tabular}{c|c|c|c|c|c}
% 	\toprule
%       \multirow{2}{*}{$\alpha$}  &\multicolumn{3}{|c|}{Loc Err.} & \multicolumn{2}{|c}{Cls Err.}  \\ 
%       \cline{2-6}
%           &Top-1 & Top-5&Gt-Known &Top-1 &Top-5 \\ \hline
%       0.0 & 54.71 & 43.35 & 38.76 & 30.60 & 10.60 \\
%       0.1 & 54.56 & 43.13 & 38.50 & 30.65 & 10.62 \\
%       0.2 & 53.97 & 42.53 & 38.05 & 30.01 & 10.15 \\
%       0.3 & 53.25 & 41.50 & 36.97 & 30.22 & 10.23 \\
%       0.4 & 53.46 & 41.43 & 37.03 & 30.93 & 10.73 \\
%       \textbf{0.5} & \textbf{52.71} & \textbf{40.82} & \textbf{36.40} & 30.19 & 10.21 \\
%       0.6 & 53.31 & 41.44 & 37.24 & 30.84 & 10.71 \\
% 	\bottomrule
% \end{tabular}
% % }
% % \caption{}
% \label{tab:ilsvrc_vgg_alpha_abl}
% }
% \end{table}


\begin{table}[!t]
\begin{minipage}[t]{0.48\linewidth}
  \centering
   \resizebox{\textwidth}{!}{
  \begin{tabular}{c|c|c|c|c|c}
	\toprule
      \multirow{2}{*}{$\alpha$}  &\multicolumn{3}{|c|}{Loc Err.} & \multicolumn{2}{|c}{Cls Err.}  \\ 
      \cline{2-6}
          &Top-1 & Top-5&Gt-Known &Top-1 &Top-5 \\ \hline
      0.0 & 54.71 & 43.35 & 38.76 & 30.60 & 10.60 \\
      0.1 & 54.56 & 43.13 & 38.50 & 30.65 & 10.62 \\
      0.2 & 53.97 & 42.53 & 38.05 & 30.01 & 10.15 \\
      0.3 & 53.25 & 41.50 & 36.97 & 30.22 & 10.23 \\
      0.4 & 53.46 & 41.43 & 37.03 & 30.93 & 10.73 \\
      \textbf{0.5} & \textbf{52.71} & \textbf{40.82} & \textbf{36.40} & 30.19 & 10.21 \\
      0.6 & 53.31 & 41.44 & 37.24 & 30.84 & 10.71 \\
	\bottomrule
  \end{tabular}
  }
  \end{minipage}
  \begin{minipage}[t]{0.48\linewidth}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{c|c|c|c|c|c}
	\toprule
      \multirow{2}{*}{$\tau$}  &\multicolumn{3}{|c|}{Loc Err.} & \multicolumn{2}{|c}{Cls Err.}  \\ 
      \cline{2-6}
          &Top-1 & Top-5&Gt-Known &Top-1 &Top-5 \\ \hline
       0.2 & 53.50 & 41.61 & 36.81 & 30.87 & 10.70 \\
       0.3 & 53.24 & 41.21 & 36.61 & 30.92 & 10.71 \\
       \textbf{0.4} & \textbf{52.71} & \textbf{40.82} & \textbf{36.40} & 30.19 & 10.21 \\
       0.5 & 52.94 & 41.46 & 37.63 & 30.18 & 10.21 \\
       0.6 & 54.95 & 44.51 & 41.98 & 30.90 & 10.73 \\
	\bottomrule
  \end{tabular}
  }
  \end{minipage}
  \begin{minipage}[t]{0.48\linewidth}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{c|c|c|c|c|c}
	\toprule
      \multirow{2}{*}{$\sigma$}  &\multicolumn{3}{|c|}{Loc Err.} & \multicolumn{2}{|c}{Cls Err.}  \\ 
      \cline{2-6}
          &Top-1 & Top-5&Gt-Known &Top-1 &Top-5 \\ \hline
       0.0 & 52.82 & 40.88 & 36.35 & 30.21 & 10.20 \\
       \textbf{0.1} & \textbf{52.71} & \textbf{40.82} & \textbf{36.40} & 30.19 & 10.21 \\
       0.2 & 53.32 & 41.52 & 37.67 & 30.89 & 10.69 \\
       0.3 & 53.53  & 42.06  &38.52  &30.86  &10.71  \\
	\bottomrule
\end{tabular}
  }
  \end{minipage}
  \vspace{-0.1cm}%设置第二个表格与正文下文的空白行距离
\end{table}


==> Tables/ilsvrc_vgg_rebuttal.tex <==
\begin{table}[!t]
%\begin{minipage}[t]{0.48\linewidth}
  \centering
%   \resizebox{\textwidth}{!}{
  \begin{tabular}{c|c|c|c||c|c|c|c}
	\toprule
	\multicolumn{4}{c||}{$M_{bg}$} & \multicolumn{4}{c}{$M_{obj}$} \\ \hline
   $\tau$(bg) & $IoU$ & $IoG$ & $IoP$ & $\tau$ + $\sigma$(fg) & $IoU$ & $IoG$ & $IoP$ \\ \hline
    0.1 & 0.42 & 0.44 & 0.92 & 0.0 &0.30 & 1.00 & 0.30 \\
    0.2 & 0.54 & 0.59 & 0.89 & 0.1 &0.33 & 1.00 & 0.33 \\
    0.3 & 0.60 & 0.69 & 0.86 & 0.2 &0.36 & 0.99 & 0.35 \\
    0.4 & 0.65 & 0.77 & 0.83 & 0.3 &0.37 & 0.98 & 0.37 \\
    0.5 & 0.67 & 0.83 & 0.80 & 0.4 &0.38 & 0.97 & 0.38 \\
    0.6 & 0.69 & 0.87 & 0.77 & 0.5 &0.38 & 0.95 & 0.40 \\
    0.7 & 0.69 & 0.90 & 0.76 & 0.6 &0.38 & 0.93 & 0.41 \\
    0.8 & 0.70 & 0.92 & 0.76 & 0.7 &0.39 & 0.90 & 0.43 \\
    0.9 & 0.71 & 0.94 & 0.75 & 0.8 &0.39 & 0.86 & 0.34 \\
	\bottomrule 
    \end{tabular}
%  }
%  \centerline{Table R1}
  \caption{Ablation study of $\tau$ and $\sigma$}
  \label{tab:sup_ablation}
%  \end{minipage}
  \end{table}
  
\begin{table}[!t]  
%  \begin{minipage}[t]{0.44\linewidth}
  \centering
%   \resizebox{\textwidth}{!}{
  \begin{tabular}{c|c|c|c|c|c}
	\toprule
      \multirow{2}{*}{$\alpha$}  &\multicolumn{3}{|c|}{Loc Err.} & \multicolumn{2}{|c}{Cls Err.}  \\ 
      \cline{2-6}
          &Top-1 & Top-5&Gt-Known &Top-1 &Top-5 \\ \hline
      0.0 & 54.71 & 43.35 & 38.76 & 30.60 & 10.60 \\
      0.1 & 54.56 & 43.13 & 38.50 & 30.65 & 10.62 \\
      0.2 & 53.97 & 42.53 & 38.05 & 30.01 & 10.15 \\
      0.3 & 53.25 & 41.50 & 36.97 & 30.22 & 10.23 \\
      0.4 & 53.46 & 41.43 & 37.03 & 30.93 & 10.73 \\
      \textbf{0.5} & \textbf{52.71} & \textbf{40.82} & \textbf{36.40} & 30.19 & 10.21 \\
      0.6 & 53.31 & 41.44 & 37.24 & 30.84 & 10.71 \\
	\bottomrule
  \end{tabular}
%  }
%  \centerline{Table R2: $\tau$=0.4,$\sigma$=0.1}
   \caption{Ablation study of $\alpha$ when fixing $\tau$=0.4, $\sigma$=0.1.}
   \label{tab:sup_abl_alpha}
%  \end{minipage}
\end{table}

\begin{table}
%  \begin{minipage}[t]{0.48\linewidth}
  \centering
%  \resizebox{\textwidth}{!}{
  \begin{tabular}{c|c|c|c|c|c}
	\toprule
      \multirow{2}{*}{$\tau$}  &\multicolumn{3}{|c|}{Loc Err.} & \multicolumn{2}{|c}{Cls Err.}  \\ 
      \cline{2-6}
          &Top-1 & Top-5&Gt-Known &Top-1 &Top-5 \\ \hline
       0.2 & 53.50 & 41.61 & 36.81 & 30.87 & 10.70 \\
       0.3 & 53.24 & 41.21 & 36.61 & 30.92 & 10.71 \\
       \textbf{0.4} & \textbf{52.71} & \textbf{40.82} & \textbf{36.40} & 30.19 & 10.21 \\
       0.5 & 52.94 & 41.46 & 37.63 & 30.18 & 10.21 \\
       0.6 & 54.95 & 44.51 & 41.98 & 30.90 & 10.73 \\
	\bottomrule
  \end{tabular}
%  }
  \caption{Ablation study of $\tau$ when fixing $\alpha$=0.5, $\sigma$=0.1.}
   \label{tab:sup_abl_tau}
%  \end{minipage}
%  \vspace{-0.4cm}
\end{table}

\begin{table}
%  \begin{minipage}[t]{0.48\linewidth}
  \centering
%  \resizebox{\textwidth}{!}{
  \begin{tabular}{c|c|c|c|c|c}
	\toprule
      \multirow{2}{*}{$\sigma$}  &\multicolumn{3}{|c|}{Loc Err.} & \multicolumn{2}{|c}{Cls Err.}  \\ 
      \cline{2-6}
          &Top-1 & Top-5&Gt-Known &Top-1 &Top-5 \\ \hline
       0.0 & 52.82 & 40.88 & 36.35 & 30.21 & 10.20 \\
       \textbf{0.1} & \textbf{52.71} & \textbf{40.82} & \textbf{36.40} & 30.19 & 10.21 \\
       0.2 & 53.32 & 41.52 & 37.67 & 30.89 & 10.69 \\
       0.3 & 53.53  & 42.06  &38.52  &30.86  &10.71  \\
	\bottomrule
\end{tabular}
%  }
    \caption{Ablation study of $\sigma$ when fixing $\alpha$=0.5, $\tau$=0.4.}
   \label{tab:sup_abl_sigma}
%   \caption*{$\alpha$=0.5,$\tau$=0.4}
%  \end{minipage}
% \vspace{-0.2cm}%设置第二个表格与正文下文的空白行距离
\end{table}

==> Tables/ilsvrc_vgg_sigma_abl.tex <==
\begin{table}[!th]
\centering
\resizebox{.23\textwidth}{!}{
% \setlength{\tabcolsep}{3.2mm}{
\begin{tabular}{c|c|c|c|c|c}
	\toprule
      \multirow{2}{*}{$\sigma$}  &\multicolumn{3}{|c|}{Loc Err.} & \multicolumn{2}{|c}{Cls Err.}  \\ 
      \cline{2-6}
          &Top-1 & Top-5&Gt-Known &Top-1 &Top-5 \\ \hline
       0.0 & 52.82 & 40.88 & 36.35 & 30.21 & 10.20 \\
       \textbf{0.1} & \textbf{52.71} & \textbf{40.82} & \textbf{36.40} & 30.19 & 10.21 \\
       0.2 & 53.32 & 41.52 & 37.67 & 30.89 & 10.69 \\
       0.3 & 53.53  & 42.06  &38.52  &30.86  &10.71  \\
	\bottomrule
\end{tabular}
% }
% \caption{}
\label{tab:ilsvrc_vgg_sigma_abl}
}
\end{table}

==> Tables/ilsvrc_vgg_tau_abl.tex <==
\begin{table}[!th]
\centering
\resizebox{.24\textwidth}{!}{
% \setlength{\tabcolsep}{3.2mm}{
\begin{tabular}{c|c|c|c|c|c}
	\toprule
      \multirow{2}{*}{$\tau$}  &\multicolumn{3}{|c|}{Loc Err.} & \multicolumn{2}{|c}{Cls Err.}  \\ 
      \cline{2-6}
          &Top-1 & Top-5&Gt-Known &Top-1 &Top-5 \\ \hline
       0.2 & 53.50 & 41.61 & 36.81 & 30.87 & 10.70 \\
       0.3 & 53.24 & 41.21 & 36.61 & 30.92 & 10.71 \\
       \textbf{0.4} & \textbf{52.71} & \textbf{40.82} & \textbf{36.40} & 30.19 & 10.21 \\
       0.5 & 52.94 & 41.46 & 37.63 & 30.18 & 10.21 \\
       0.6 & 54.95 & 44.51 & 41.98 & 30.90 & 10.73 \\
	\bottomrule
\end{tabular}
% }
% \caption{}
\label{tab:ilsvrc_vgg_tau_abl}
}
\end{table}
